Quadratic Zonotopes:An extension of Zonotopes to Quadratic Arithmetics

Affine forms are a common way to represent convex sets of $\mathbb{R}$ using a base of error terms $\epsilon \in [-1, 1]^m$. Quadratic forms are an extension of affine forms enabling the use of quadratic error terms $\epsilon_i \epsilon_j$. In static analysis, the zonotope domain, a relational abstract domain based on affine forms has been used in a wide set of settings, e.g. set-based simulation for hybrid systems, or floating point analysis, providing relational abstraction of functions with a cost linear in the number of errors terms. In this paper, we propose a quadratic version of zonotopes. We also present a new algorithm based on semi-definite programming to project a quadratic zonotope, and therefore quadratic forms, to intervals. All presented material has been implemented and applied on representative examples.

==> README <==
To create the paper:
in experiments folder:
./run_benchmarks.sh run_all_tex > results_apron.tex
then in paper folder:
cat ../experiments/results_apron.tex | sed "s/_/\\\\_/g;s/\(\.[0-9][0-9]\)[0-9]*/\1/g;s/e+\([0-9]*\)/e^{+\1}/g;s/, /,\\\\allowbreak /g" > runs_apron.tex


==> computable_po.tex <==
\section{Computable partial order}
\label{sec-4}
\ploc{Est-ce qu'on garde cette section?}

The presented result show the interest of quadratic forms and their zonotopic
extension when performing static analysis based on environement updates with
arithmetic expressions, contraints over zonotopes, and join of
zonotopes. However it does not consider any framework relying on the use of the
partial order such as any simple Kleene iteration schema.

We present now an alternative partial order for $\A$ and $\Q$ and show that a
similar hierarchy of abstraction occurs. This motivate again the use of
quadratic zonotopes in lieu of classical ones.

A first definition characterize the new partial order over elements of $\A$. It
is inspired by\cite{goubault} but \ploc{...}.

\begin{definition}[$\sqsubseteq^\#_\A$]
\ploc{todo}
\end{definition}

\begin{definition}[$\sqsubseteq^\#_\Q$]
\ploc{todo}
\end{definition}

All other operators are kept the same. We have to ensure that all theorem still
apply.
\ploc{Est ce que c'est le meme join? (argmin)}

proofs
\begin{itemize}
\item soundness of $\sqcup_\A$ (it is a join)
\item soundness of $\sqcup_\Q$ (it is a join)
\item galois connection $\AQ$
\end{itemize}
\ploc{regarder si l'ordre partiel sert dans les preuves. Si non, dire que les
preuves sont pas impactées.}


We have now the following hierarchy of abstractions using zonotopes.
\begin{itemize}
\item dessins avec 
  $\wp(\mathbb{R}, \langle \ZA{p}{n}, \sqsubseteq\rangle, \Q, \ZA{p}{n}, \ZQ{p}{n}$
\end{itemize}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "submission"
%%% End: 


==> preuve_proposition_bounds.tex <==
\begin{proof}
\label{proofboundsimprov}
We only prove the proposition for the upper bounds, the proof for the lower bounds can be done similarly. 
Let $X\succeq 0$ be in $\CCm$. We can write $X$ as a the following block matrix (the notations around the matrix indicates the sizes of the blocks):

\vspace{8pt}

\[
\begin{array}{cl}\multirow{3}{*}{
$\begin{pmatrix}\noalign{\vspace{-20pt}}
m & 3 & 1 \\[-3pt]
\overbrace{} & \overbrace{} & \overbrace{} \\
X^A & X^0 & X^b \\
{X^0}^\intercal & X^{00} & X^c\\
{X^b}^\intercal & {X^c}^\intercal & 1 
\end{pmatrix}$} &\big\} m\\
&\big\} 3\\
&\big\} 1\\
\end{array}
\]
Recall that $\tr$ is linear and satisfies for all square matrices $M$, $\tr(M^\intercal)=\tr(M)$ and for all matrices $A,B$ such that 
$AB$ and $BA$ are square matrices, $\tr(AB)=\tr(BA)$. Considering this and the symmetry of $X$, we have after simplifications: 
$\tr\left(\Mat^{r_q} X\right)=\tr\left(A^q X^{A}\right)+{b^q}^\intercal X^{b}+{X^{c}}^\intercal (c_{\pm},c_+,c_-)+c^q$.
Constraints~\eqref{eq_cont:1} and~\eqref{eq_cont:3} yield to $\tr\left(A^q X^{A}\right)\leq \sum_{i=1}^m \sum_{\substack{j=1,\ldots,m\\ j\neq i}} \left|(A^q)_{i,j}\right|+\sum_{i=1}^m [(A^q)_{i,i}]^+$. Constraint~\eqref{eq_cont:2} implies that ${b^q}^\intercal X^{b_q}\leq \sum_{j=1}^{m} \left|{b^q}_{j}\right|$ and Constraints~\eqref{eq_cont:4} and~\eqref{eq_cont:5} imply that ${X^{c}}^\intercal (c_{\pm},c_+,c_-)\leq c_{\pm}+c_+$. By summation, we conclude that $\tr\left(\Mat^{r_q} X\right)\leq \mathbf{B}^q_{MT}$ for all $X\succeq 0$ in $\CCm$ and then $\mathbf{B}^q_{SDP}\leq \mathbf{B}^q_{MT}$. 
\end{proof}


==> preuve_theorem1.tex <==
\begin{proof}[Proof of Theorem~\ref{thjoin}]
\label{proofthjoin}
We only prove that $q\sqsubseteq_{\ZQ{}{}} q \sqcup_{\ZQ{}{}} q'$. Let for all $k\in [p]$, $r_k=\ext_{m+p}(q_k)-q_k''$ and $r'_k=\ext_{m+p}(q'_k)-q_k''\in\Q^{m+p}$. 
By Lemma~\ref{lemmajoin}, it suffices to show that for all $t\in \ccm$, it exists $t^\sharp\in\ccmp$ such that for all $k\in [p]$ 
$q_k(t)-q''_k(t^\sharp)\in \gamma_{\Q^{m+p}}(q_k^{err})$ i.e.
$\min(\mathbf{b}^{r_k},\mathbf{b}^{r'_k})
\leq q_k(t)-q''_k(t^\sharp)$ and $\max(\mathbf{B}^{r_k},\mathbf{B}^{r'_k})
\geq q_k(t)-q''_k(t^\sharp)$.
Let $t=(\epsilon,\epsilon_{\pm},\epsilon_+,\epsilon_-)\in \ccm$ and let us define $\epsilon^\sharp\in[-1,1]^{m+p}$ such that for all $i\in [m+p]$, $\epsilon_i^\sharp=\epsilon_i$ if $i\in [m]$ and 0 otherwise and 
$t^\sharp=(\epsilon^\sharp,\epsilon_{\pm},\epsilon_+,\epsilon_-)$, we have for all $k\in [p]$,  
$\min(\mathbf{b}^{r_k},\mathbf{b}^{r'_k})\leq\mathbf{b}^{r_k} \leq \ext_{m+p}(q_k)(t^\sharp)-q''_k(t^\sharp)=q_k(t)-q''_k(t^\sharp)$. The same argument holds for the upper bound and the conclusion follows.
\end{proof}


==> quadformgalois.tex <==
\section{Affine arithmetics as an abstraction of Quadratic arithmetics: the unidimensional case}
\label{sec-2}


In a first step we only consider single dimension zonotopes, ie. forms. We would
like to show that quadratic forms are always more precise, with respect to the
geometric interpretation, than affine ones.

Let us first formally define the poset structure associated to this set
$\Q$:

\begin{definition}[Geometrical Inclusion based Partial Order for $\Q$]
\label{def:orderQ}
We define the partial order $\sqsubseteq_\Q: \Q \times
\Q \rightarrow \mathbb{B}$ such that:
\[
\forall x,y \in \Q, x \sqsubseteq_\Q y \triangleq
\gamma_\Q (x) \subseteq \gamma_\Q (y)
\]
\end{definition}

% The join operator $\sqcup_\Q$ computes the algorithm of the join
% $\sqcup_\A$ (cf. Eq. (\ref{eq:joinA})) considering quadratic terms in
% $\epsilon_i\epsilon_j$ as new terms.

% \begin{definition}[Join in $\Q$]
% \alexis{reprendre la def formelle de $\sqcup_\A$ et l'adapter au cas quadratique.}
% \end{definition}

% \begin{property}[Join soundness]
% $\sqcup_\Q: \Q \times \Q \rightarrow \Q$
% is a sound join with respect to the poset $\langle \Q, \sqsubseteq\\Q \rangle$.
% \end{property}

% \begin{proof}
% \ploc{utiliser la def du join}
% \end{proof}

We now consider our pair of conversion functions $(Conv_{\QA},
Conv_{\AQ})$ where $Conv_{\QA}$, the abstraction function,
maps a quadratic form to an affine form and $Conv_{\AQ}$, the
concretization function, maps an affine form to a quadratic one.
In the following, we denote respectively by $\alpha_{\AQ}$ and $\gamma_{\AQ}$
the abstraction and concretization functions $Conv_{\QA}$ and $Conv_{\AQ}$.


\begin{theorem}
The pair $(\alpha_{\AQ},\gamma_{\AQ})$ is a Galois connection:
 \[\langle\Q, \sqsubseteq_\Q \rangle  \galoisconn{\AQ} \langle \A, \sqsubseteq_\A\rangle\]
\end{theorem}

\begin{proof}
\begin{itemize}
\item $\gamma_{\AQ}$ is monotonic: $\forall (c,(b)_m), (c,(b')_m) \in \A$, if
  $(c,(b)_m) \sqsubseteq_\A (c',(b')_m)$ then, using Def.\ref{def:orderA} of
  $\sqsubseteq_\A$, $\gamma_\A (c,(b)_m) \subseteq \gamma_\A (c',(b')_m)$, and
  using Def.\ref{def:gammaA} of $\gamma_\A$, $\left\{ c + b^\intercal \epsilon
    \mid \epsilon \in [-1;1]^m \right\} \subseteq \left\{ c' + b'^\intercal
    \epsilon \mid \epsilon \in [-1;1]^m \right\}$.  
  %
  By
  Defs~\ref{def:orderQ},\ref{def:gammaQ},\ref{def:gammaAQ},
  $\gamma_{\AQ}((c,(b)_m)) \sqsubseteq_\Q \gamma_{\AQ}((c',(b')_m))$ iff
  $\left\{ c + b^\intercal \epsilon + \epsilon^\intercal 0_{m^2} \epsilon \mid
    \epsilon \in [-1;1]^m \right\} \subseteq \left\{ c' + b'^\intercal
    \epsilon + \epsilon^\intercal 0_{m^2} \epsilon \mid \epsilon \in [-1;1]^m
  \right\}$. 
\item $\alpha_{\AQ}$ is monotonic: let us first show that $\forall q \in \Q,
  \gamma_\Q(q) = \gamma_\A \circ \alpha_\AQ (q)$. 


Then, using the definition of $\sqsubseteq_\Q$ (Def~\ref{def:orderQ}), the bound
preservation corollary and the definition of $\sqsubseteq_\A$
(Def~\ref{def:orderA}), we have $\forall q,q' \in \Q, q \sqsubseteq_\Q q'
\implies \alpha_\AQ(q) \sqsubseteq_\A \alpha_\AQ(q')
 assume that $\forall q = (c,(b)_m,
  (A)_{m^2}, c_\pm, c_+, c_-),$ $q' = (c',(b')_m, (A')_{m^2}, c'_\pm, c'_+, c'_-) \in
  \Q$, if $q \sqsubseteq_\Q  q'$ then, by Defs. \ref{def:orderQ},
  \ref{def:gammaQ}, $\left\{ x \in \mathbb{R} \left|
      \begin{array}{l}
        \exists \epsilon \in
        [-1;1]^m, \epsilon_\pm \in [-1;1], \epsilon_+ \in
        [0;1], \epsilon_- \in [-1, 0]\\ \textrm{ s.t. } x = c + b^\intercal \epsilon +
        \epsilon^\intercal A \epsilon + c_\pm \epsilon_\pm + c_- \epsilon_- +
        c_+ \epsilon_+
\end{array}
      \right\}\right. \subseteq 
\left\{ x \in \mathbb{R} \left|
      \begin{array}{l}
        \exists \epsilon \in
        [-1;1]^m, \epsilon_\pm \in [-1;1], \epsilon_+ \in
        [0;1], \epsilon_- \in [-1, 0]\\ \textrm{ s.t. } x = c' + b'^\intercal \epsilon +
        \epsilon^\intercal A' \epsilon + c'_\pm \epsilon_\pm + c'_- \epsilon_- +
        c'_+ \epsilon_+
\end{array}
      \right\}\right.
$
Let us consider now the set 
$\gamma_\A \circ \alpha_{\AQ}(q) =  \left\{ x \in \mathbb{R} \mid \exists \epsilon \in
        [-1;1]^{m+1}, \textrm{ s.t. } x = c + b^\intercal \epsilon_{1\leq i \leq
          m}+ max \left\{
  \begin{array}{l}
    -\left( \sum_{i,j\in [1,m]} |A_{i,j}| + c_\pm + c_-\right),\\
    \sum_{i,j\in [1,m]}  |A_{i,j}| + c_\pm + c_+
                      \end{array}
\right\} \epsilon_{m+1} \right\}$. 

Assume now that $\alpha_{\AQ}(q) \sqsubsetneq_\A \alpha_{\AQ}(q')$. Then
according to Defs.~\ref{def:alphaAQ},\ref{def:orderA},\ref{def:gammaA}, 

$\left\{ x \in \mathbb{R} \mid \exists \epsilon \in
        [-1;1]^{m+1}, \textrm{ s.t. } x = c + b^\intercal \epsilon_{1\leq i \leq
          m}+ max \left\{
  \begin{array}{l}
    -\left( \sum_{i,j\in [1,m]} |A_{i,j}| + c_\pm + c_-\right),\\
    \sum_{i,j\in [1,m]}  |A_{i,j}| + c_\pm + c_+
                      \end{array}
\right\} \epsilon_{m+1} \right\}$

$\left\{
\begin{array}{l}
\left(c,(b')_{m+1}\right) \textrm{ where}\\
\forall i \in [1;m], b'_i = b_i\\
b'_{i+1} = max \left\{
  \begin{array}{l}
    -\left( \sum_{i,j\in [1,m]} |A_{i,j}| + c_\pm + c_-\right),\\
    \sum_{i,j\in [1,m]}  |A_{i,j}| + c_\pm + c_+
                      \end{array}
\right\}
\end{array}
\right.$
\alexis{il manque la def d'alpha}
\item $\alpha_{\AQ} \circ \gamma_{\AQ}$ is reductive: $\forall (c,(b)_m)  \in \A, \alpha_{\AQ} \circ \gamma_{\AQ} ((c,(b)_m)) = \alpha_{\AQ} ((c,(b)_m,0_{m^2})) = (c, (b)_m)$.
\item $\gamma_{\AQ} \circ \alpha_{\AQ}$ is extensive: \alexis{\textrm{ besoin def alpha}}
\end{itemize}
\end{proof}

We now have to prove the soundness of the domain operators over affine form
with respect to the Galois connection.

% \begin{theorem}[Join soundness]
% The join in $\A$ is a monotonic function, sound overapproximation 
% of the join in $\Q$.
% \[
% \forall a,b \in \A,
% \left\{
% \begin{array}{l}
%  \alpha_{\AQ}\left(\gamma_{\AQ}(a)
% \sqcup_\Q \gamma_{\AQ}(b)\right) \sqsubseteq_\A a \sqcup_\A b\\
% a \sqsubseteq_\A a \sqcup_\A b\\
% b \sqsubseteq_\A a \sqcup_\A b
% \end{array}
% \right.
% \]
% \end{theorem}

% \begin{proof}
% Since the concretization $\gamma_{\AQ}$ produces a quadratic form with 
% a null quadratic part, the join $\sqcup_\Q$ in $\Q$ coincides
% with the join $\sqcup_\A$ in $\A$. 
% The abstraction $\alpha_{\AQ}$ applied to the resulting quadratic form 
% with an empty quadratic part generates an affine form without the additional error term. 
% Then $\alpha_{\AQ}\left(\gamma_{\AQ}(a) \sqcup_\Q 
% \gamma_{\AQ}(b)\right) = a \sqcup_\A b$. 
% It is an exact approximation of $\sqcup_\Q$.
% \end{proof}

\begin{theorem}[Addition soundness]
The addition in $\A$ is a sound overapproximation of the addition in $\Q$. \[\forall a,b \in \A, \alpha_{\AQ}\left(\gamma_{\AQ}(a) +_\Q \gamma_{\AQ}(b)\right) \sqsubseteq_\A a +_\A b\]
\end{theorem}

\begin{proof}
Since the concretization $\gamma_{\AQ}$ produces a quadratic form with a null quadratic part, the addition $+_\Q$ in $\Q$ coincides with the addition $+_\A$ in $\A$. The abstraction $\alpha_{\AQ}$ applied to the resulting quadratic form with an empty quadratic part generates an affine form without the additional error term. 
Then $\alpha_{\AQ}\left(\gamma_{\AQ}(a) +_\Q \gamma_{\AQ}(b)\right) = a +_\A b$. It is an exact approximation.
\end{proof}

\begin{theorem}[Negation soundness]
The negation in $\A$ is a sound overapproximation of the negation in
$\Q$. \[\forall a \in \A, \alpha_{\AQ}\left(-_\Q \gamma_{\AQ}(a)a \right)
\sqsubseteq_\A -_\A a \]
\end{theorem}

\begin{theorem}[Scalar multiplication soundness]
\[\forall a \in \A, \lambda \in \mathbb{R}, \lambda *_\Q \left( \gamma_{\AQ}(a)\right) \sqsubseteq_\A \lambda *_\A a\]
\end{theorem}

\begin{proof}
Similarly, since the concretization $\gamma_{\AQ}$ produces a quadratic form with a null quadratic part, $\alpha_{\AQ}$ zill not introduce an additional error term and the two operators $*_\Q$ and $*_\A$ coincides:
$\forall (c,(b)_m) \in \A, \lambda *_\Q (\gamma_{\AQ} ((c,(b)_m))) = \lambda *_\Q ((c,(b)_m, 0_{m^2})) = ((\lambda c,\lambda (b)_m, 0_{m^2}))$. 
Then $\alpha_{\AQ}\left(\lambda *_\Q \gamma_{\AQ}(a)\right) = \lambda *_\A a$. It is an exact approximation.
\end{proof}

\begin{theorem}[Multiplication soundness]
\[\forall a,b \in \A, \alpha_{\AQ}\left(\gamma_{\AQ}(a) \times_\Q \gamma_{\AQ}(b)\right) \sqsubseteq_\A a \times_\A b\]
\end{theorem}

\begin{proof}
\alexis{manque def multiplication}.
\end{proof}

\begin{theorem}
$\langle \A, \sqsubseteq_\A, \sqcup_\A, +_\A, 
\times_\A, *_\A \rangle$ is a sound over-approximation of $\langle \Q, \sqsubseteq_\Q, \sqcup_\Q, +_\Q, 
\times_\Q, *_\Q \rangle$. 
\end{theorem} 


\begin{remark}
Let us remark that the geometrical concretization usually associated to affine
form, $\gamma_\A$, is exactly $\gamma_\Q \circ \gamma_\AQ$.
\end{remark}

\begin{proof}
Using definitions\ref{gammaA,gammaQ,gammaAQ}.
\end{proof}

We exhibited a Galois connection between quadratic arithmetics and affine
arithmetics and showed the soundness of their respective operators. This
guaranty that the use of quadratic arithmetic will always to lead to values at
least as precise as the ones obtained with affine arithmetics. Here ``precise''
means geometrically included.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "submission"
%%% End: 


==> quadzongalois.tex <==

\section{Affine Zonotopes as an abstraction of Quadratic Zonotopes}
\label{sec:zongalois}

decoupage a revoir


idem: 
\subsection{galois connection sur l'extension n dimensionnelle}
\label{sec-3-1}

\begin{itemize}
\item alpha
\end{itemize}
-gamma
\begin{itemize}
\item monotonie alpha
\item monotonie gamma
\item prove reductivity/extensivity
\end{itemize}
\subsection{soundness}
\label{sec-3-2}

\begin{itemize}
\item constrain
\item assign
\end{itemize}
\subsection{New operator:}
\label{sec-3-3}

\begin{itemize}
\item infeq? definition dans Q
\item join? definition dans Q - illustration
\item preuve correction de infeq$_Q$ par rapport a wp(R)
\item preuve correction de join$_Q$ par rapport a wp(R)
\item preuve correction de infeq$_A$ par rapport a infeq$_Q$
\item preuve correction de join$_A$ par rapport a join$_Q$
\end{itemize}
 
\subsection{Galois connexion - Hiearchy of abstraction : R$^n$ - Q$^n$ - Z$^n$}
\label{sec-3-4}

super!

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "submission"
%%% End: 


==> runs.tex <==
atan
& [-1.91, 1.91] & 3
& [-1.91, 1.91] & 9
& \best{[-1.00, 1.00]} & 0
\\
atan10
& [-1.91, 1.91] & 9
& [-2.36, 2.36] & 12
& \best{[-1.59, 1.59]} & 7
\\
stolfi1
& [0., \infty] & 7
& [-\infty, +\infty] & 0
& \best{[-0.85, 3.25]} & 5
\\
stolfi2
& \best{[0., 3.60]} & 0
& [-\infty, +\infty] & 0
& [-\infty, +\infty] & 0
\\
stolfi3
& [0., 5.38] & 3
& [-2.98, 10.81] & 9
& \best{[-0.62, 3.24]} & 4
\\
stolfi4
& \best{[0., 2.23]} & 4
& [-\infty, +\infty] & 4
& [-0.33, 3.26] & 6
\\
stolfi5
& \best{[0., 2.18]} & 0
& [-0.42, 3.03] & 7
& [0.08, 2.38] & 7
\\
stolfi6
& \best{[0., 2.18]} & 4
& [-0.71, 2.91] & 3
& [0.11, 2.30] & 6
\\
stolfi7
& [0., 1.89] & 5
& [0.19, 2.23] & 7
& \best{[0.29, 1.97]} & 7
\\
stolfi8
& [-0., 1.82] & 3
& [0.20, 2.] & 11
& \best{[0.29, 1.88]} & 3
\\
stolfi9
& [0., 1.73] & 0
& [0.26, 1.89] & 2
& \best{[0.33, 1.75]} & 3
\\
stolfi10
& [0., 1.71] & 8
& [0.32, 1.82] & 7
& \best{[0.36, 1.75]} & 7
\\
stolfi11
& [0., 1.67] & 3
& [0.34, 1.74] & 6
& \best{[0.39, 1.67]} & 7
\\
stolfi13
& [0., 1.61] & 0
& [0.38, 1.67] & 7
& \best{[0.41, 1.61]} & 5
\\
stolfi30
& [0.35, 1.43] & 11
& [0.48, 1.44] & 16
& \best{[0.48, 1.43]} & 10
\\
stolfi40
& [0.40, 1.40] & 13
& [0.49, 1.40] & 19
& \best{[0.50, 1.40]} & 15
\\
stolfi50
& [0.43, 1.38] & 17
& [0.50, 1.38] & 25
& \best{[0.50, 1.38]} & 25
\\
stolfi55
& [0.44, 1.37] & 16
& [0.51, 1.37] & 31
& \best{[0.51, 1.37]} & 23
\\
stolfi100
& [0.48, 1.34] & 25
& [0.52, 1.34] & 67
& \best{[0.52, 1.34]} & 56
\\
stolfi200
& [0.51, 1.32] & 46
& [0.53, 1.32] & 267
& \best{[0.53, 1.32]} & 210
\\
stolfi300
& [0.52, 1.31] & 57
& [0.53, 1.31] & 714
& \best{[0.53, 1.31]} & 430
\\
stolfi400
& [0.52, 1.31] & 74
& [0.53, 1.31] & 1370
& \best{[0.53, 1.31]} & 863
\\
Ln1px
& [-0.00, 0.46] & 0
& [-0.00, 0.40] & 4
& \best{[-0.00, 0.40]} & 0
\\
householder\_orig
& \best{[0.11, 0.11]} & 4
& [0.11, 0.11] & 8
& [0.11, 0.11] & 0
\\
householder\_orig
& [0.17, 0.18] & 6
& [0.17, 0.18] & 3
& \best{[0.17, 0.18]} & 5
\\
householder\_orig
& [0.21, 0.24] & 5
& [0.21, 0.24] & 10
& \best{[0.21, 0.24]} & 10
\\
householder\_orig
& [0.17, 0.29] & 3
& [0.22, 0.25] & 4
& \best{[0.22, 0.24]} & 2
\\
householder\_orig
& [0.03, 0.42] & 4
& [0.22, 0.25] & 15
& \best{[0.22, 0.24]} & 7
\\
householder\_orig
& [-0.90, 1.66] & 6
& [0.22, 0.25] & 20
& \best{[0.22, 0.24]} & 4
\\
householder\_orig
& [-1117.82, 1899.48] & 5
& [0.22, 0.25] & 34
& \best{[0.22, 0.24]} & 6
\\
householder\_orig
& [-2.18e^{+18}, 3.70e^{+18}] & 4
& [0.22, 0.25] & 16
& \best{[0.22, 0.24]} & 3
\\
householder\_orig
& [-6.19e^{+94}, 1.05e^{+95}] & 3
& [0.22, 0.25] & 32
& \best{[0.22, 0.25]} & 7
\\
householder\_orig
& [-\infty, \infty] & 6
& [0.22, 0.25] & 37
& \best{[0.22, 0.25]} & 4
\\
householder\_orig
& [-\infty, \infty] & 2
& [0.22, 0.25] & 36
& \best{[0.22, 0.25]} & 11
\\
householder\_orig
& [-\infty, \infty] & 10
& [0.22, 0.25] & 33
& \best{[0.22, 0.25]} & 2
\\
householder\_orig
& [-\infty, \infty] & 4
& [0.22, 0.25] & 27
& \best{[0.22, 0.25]} & 6
\\
householder\_orig
& [-\infty, \infty] & 6
& [0.22, 0.25] & 23
& \best{[0.22, 0.25]} & 4
\\
householder\_orig
& [-\infty, \infty] & 3
& [0.22, 0.25] & 23
& \best{[0.22, 0.25]} & 6
\\
householder\_orig
& [-\infty, \infty] & 4
& \best{[0.22, 0.25]} & 18
& [0.23, 0.26] & 0
\\
householder\_orig
& [-\infty, \infty] & 0
& \best{[0.22, 0.25]} & 18
& [0.24, 0.27] & 13
\\
householder
& \best{[0.11, 0.11]} & 3
& [0.11, 0.11] & 0
& [0.11, 0.11] & 0
\\
householder
& [0.17, 0.18] & 4
& [0.17, 0.18] & 5
& \best{[0.17, 0.18]} & 3
\\
householder
& [0.21, 0.24] & 0
& [0.21, 0.24] & 11
& \best{[0.21, 0.24]} & 5
\\
householder
& [0.17, 0.29] & 0
& [0.21, 0.25] & 7
& \best{[0.22, 0.25]} & 0
\\
householder
& [0.03, 0.42] & 3
& [0.20, 0.26] & 10
& \best{[0.21, 0.25]} & 21
\\
householder
& [-0.90, 1.66] & 4
& [0.19, 0.27] & 8
& \best{[0.21, 0.25]} & 11
\\
householder
& [-1117.82, 1899.48] & 7
& [0.17, 0.29] & 12
& \best{[0.21, 0.25]} & 11
\\
householder
& [-2.18e^{+18}, 3.70e^{+18}] & 3
& [0.12, 0.34] & 13
& \best{[0.21, 0.25]} & 16
\\
householder
& [-6.19e^{+94}, 1.05e^{+95}] & 0
& [-0.16, 0.64] & 15
& \best{[0.21, 0.26]} & 12
\\
householder
& [-\infty, \infty] & 6
& [-14.08, 14.55] & 8
& \best{[0.20, 0.26]} & 11
\\
householder
& [-\infty, \infty] & 6
& [-98003775.36, 98003775.83] & 11
& \best{[0.20, 0.27]} & 18
\\
householder
& [-\infty, \infty] & 2
& [-1.35e^{+42}, 1.35e^{+42}] & 8
& \best{[0.18, 0.30]} & 14
\\
householder
& [-\infty, \infty] & 4
& [-6.88e^{+212}, 6.88e^{+212}] & 7
& \best{[0.15, 0.35]} & 14
\\
householder
& [-\infty, \infty] & 9
& [-\infty, +\infty] & 10
& \best{[0.04, 0.52]} & 16
\\
householder
& [-\infty, \infty] & 10
& [-\infty, +\infty] & 8
& \best{[-1.41, 2.27]} & 19
\\
householder
& [-\infty, \infty] & 9
& [-\infty, +\infty] & 10
& \best{[-2570.28, 2582.02]} & 12
\\
householder
& [-\infty, \infty] & 0
& [-\infty, +\infty] & 15
& \best{[-2.85e^{+18}, 2.85e^{+18}]} & 20
\\
householder
& [-\infty, \infty] & 3
& [-\infty, +\infty] & 16
& \best{[-4.62e^{+93}, 4.62e^{+93}]} & 20
\\
controller
& [-0.21, 0.21] & 8
& \best{[-0.15, 0.15]} & 45
& \best{[-0.15, 0.15]} & 20
\\
controller
& [-0.42, 0.42] & 16
& \best{[-0.19, 0.19]} & 191
& \best{[-0.19, 0.19]} & 24
\\
controller
& [-0.65, 0.65] & 27
& \best{[-0.20, 0.20]} & 499
& \best{[-0.20, 0.20]} & 38
\\
controller
& [-1.25, 1.25] & 30
& \best{[-0.23, 0.23]} & 1853
& \best{[-0.23, 0.23]} & 92
\\
SinCos
& [0.86, 1.18] & 10
& [0.99, 1.01] & 6
& \best{[0.99, 1.00]} & 6
\\


==> stateofart.tex <==


\subsection{State of the art}
\label{sec:soa}

We present here the two roots of this work: one the one hand related works in
the static analysis community focused on the use of affine arithmetics to
analyze programs, then on the other hand the quadratic extension of affine
arithmetics.

\ploc{
on presente les formes affines et quad
pour les zonotopes on dit:
- c'est un domaine relationnel pas cher: un relationnel parametric 
  la structure est non realtionnel:
  assign c'est l'eval dans A et la substitution dans l'env
  guard c'est l'utilisation d'op avant et arriere comme dans [cousot]
  attention pas  de structure de treillis: union zonotopique et meet pointwise
  via concretization interval
  en gros: meet pourri, union pas top

  travaux de khalil pour ameliorer le meet


puis une sectio nformal preliminaries avec les def
affine
quad
join et meet ZA

}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "submission"
%%% End: 

